Exploring Constraint Handling Techniques in Real-world Problems on MOEA/D with Limited Budget of Evaluations

Finding good solutions for Multi-objective Optimization (MOPs) Problems is considered a hard problem, especially when considering MOPs with constraints. Thus, most of the works in the context of MOPs do not explore in-depth how different constraints affect the performance of MOP solvers. Here, we focus on exploring the effects of different Constraint Handling Techniques (CHTs) on MOEA/D, a commonly used MOP solver when solving complex real-world MOPs. Moreover, we introduce a simple and effective CHT focusing on the exploration of the decision space, the Three Stage Penalty. We explore each of these CHTs in MOEA/D on two simulated MOPs and six analytic MOPs (eight in total). The results of this work indicate that while the best CHT is problem-dependent, our new proposed Three Stage Penalty achieves competitive results and remarkable performance in terms of hypervolume values in the hard simulated car design MOP.

==> files/moonHV_table.tex <==
\begin{table}[htb]
\centering
	\normalsize
	\caption{MOON experiments Hypervolume}
	\label{chap4:moon_hv_table}
    \begin{tabular}{|l|l|}
        \hline
        \rowcolor[gray]{.85}CHT                             & Mean HV   \\ \hline
        No penalty                                          & $0.05677023 \pm  0.1800290$     \\ \hline
        Static Penalty                                      & $0.24428512 \pm 0.3207784$     \\ \hline
        Superiority of Feasible Solutions                   & $0.19445319 \pm 0.1000375$     \\ \hline
        Multistaged                                         & $0.34783825 \pm 0.3406727$     \\ \hline
        Dynamic Penalty (Slow growth)                       & $0.30906154 \pm 0.3337374$     \\ \hline
        Dynamic Penalty (Fast growth)                       & $0.40948633 \pm 0.3059798$     \\ \hline
        Selfadaptive                                        & $0.12061820 \pm 0.2328939$     \\ \hline
        Three Stage Penalty                                 & $0.29991636 \pm 0.3089084$     \\ \hline
        
                                                            
\end{tabular}
\end{table}

%3stageNEW  dynamicC002alpha2   dynamicC005alpha2   multistaged     none        selfadapting    static1     static1000
%0.29991636 0.30906154          0.40948633          0.34783825      0.05677023  0.12061820      0.24428512  0.19445319
%0.3089084  0.3337374           0.3059798           0.3406727       0.1800290   0.2328939       0.3207784   0.1000375
